Effective Quantum Spacetimes from Functional Renormalization Group

Using the Functional Renormalization Group approach we construct effective quantum spacetime geometries by self-consistently deforming the classical Schwarzschild-de Sitter black-hole solution. This involves studying how quantum corrections, driven by the running of the Newton's and cosmological constants modify the solution across the infrared and ultraviolet regimes. We show that these quantum modifications replace the Schwarzschild singularity with a milder conical one. Moreover, two new features emerge in the ultraviolet regime. First, we identify a phase transition between Anti-de Sitter/de Sitter spacetime occurring when the object's mass exceeds a first critical threshold. Second, we predict the formation of horizons once the object's mass exceeds a second threshold. Both thresholds are of the order of the Planck mass. Finally, we investigate the role of the anomalous dimension in the conformal sector of the theory.

==> LetterResponceReferee.tex <==
Dear Editor of PRD,

We thank the referee for having reviewed our paper and for his/her suggestions and useful comments, 
which enabled us to improve our manuscript. In the present version, we have addressed all the issues raised by the referee and changed the manuscript accordingly. 

Our response to the referee's queries and the changes made to the manuscript  
are between brackets >>...<<.

Best regards, 
Alfio Bonanno
Mariano Cadoni
Mirko Pitzalis
Andrea Pierfrancesco Sanna

----------------------------------------------------------------------
Report of the Referee -- DX13738/Bonanno
----------------------------------------------------------------------

The paper offers a consistent treatment of a renormalization group
(RG) improved black hole spacetime based on a matching between a
radial proper distance and the RG scale k. The findings are based on
equation (11). The properties of the resulting black holes are
examined and compared to the classical Schwarzschild solution. An
interesting result is that the latter's central singularity is
replaced by a weaker conical singularity.

However, one feature of (11) is that the derivative of the proper
distance, hence the derivative of k(r) is singular when the lapse
function vanishes. This means that the black hole spacetimes are
singular at the horizon. In particular, one expects a curvature
singularity on the horizons of the effective black hole space-time (no
matter how large the mass). This important aspect is not discussed.
Even though the central singularity is weakened, the existence of a
curvature singularity on the horizon seems surprising and calls into
question the use of (11) to arrive at an effective description of
quantum geometry.

>> We thank the referee for highlighting this important aspect, which was not fully addressed in the original version of the paper. In response, we have added subsection V E, titled "Regularity of Event Horizons", where we quote the relevant literature on the subject (we have added Refs. (29) and (30)), discuss the regularity of our black-hole models at event horizons in details and check the regularity of the curvature invariants at the black-hole horizons. 
Specifically, we have calculated the dimensionless curvature invariants at the event horizons of our numerical solutions, focusing on the parameter region where our solutions were obtained using the shooting method. In our analysis, we focused on a two-horizon and an extremal solutions, reporting the plots of the curvature invariants in the new figs. 6 and 7. We have also improved the numerical computations of the extremal solution in fig. 5 (black solid line) and recalculated (41) accordingly.

We were unable to determine the functional form of the metric function in the near-horizon region. However, we argue that the behaviour of the metric function there must have a quite non-trivial, non analytic behaviour, which differs significantly from Schwarzschild or any quantum-deformed version thereof.

In the conclusions, we have added some comments briefly mentioning possible phenomenological implication of our results, in particular for black holes with astrophysical mass. <<

This point must be properly discussed before the paper can be
published.

>>  We have amended our manuscript according to the critical remarks of the referee. We hope it is now suitable for publication. <<
